Adjoint Orbits of Matrix Groups over Finite Quotients of Compact Discrete Valuation Rings and Representation Zeta Functions

This paper gives methods to describe the adjoint orbits of $\mathbf{G}(\mathfrak{o}_r)$ on $\mathrm{Lie}(\mathbf{G})(\mathfrak{o}_r)$ where $\mathfrak{o}_r=\mathfrak{o}/\mathfrak{p}^r$ ($r\in\mathbb{N}$) is a finite quotient of the localization $\mathfrak{o}$ of the ring of integers of a number field at a prime ideal $\mathfrak{p}$ and $\mathbf{G}$ is a closed $\mathbb{Z}$-subgroup scheme of $\mathrm{GL}_{n}$ for an $n\in\mathbb{N}$ and such that the Lie ring $\mathrm{Lie}(\mathbf{G})(\mathfrak{o})$ is quadratic.. The main result is a classification of the adjoint orbits in $\mathrm{Lie}(\mathbf{G})(\mathfrak{o}_{r+1})$ whose reduction $\bmod\,\mathfrak{p}^{r}$ contains $a\in\mathrm{Lie}(\mathbf{G})(\mathfrak{o}_r)$ in terms of the reduction $\bmod\mathfrak{p}$ of the stabilizer of $a$ for the $\mathbf{G}(\mathfrak{o}_r)$-adjoint action. As an application, this result is then used to compute the representation zeta function of the principal congruence subgroups of $\mathrm{SL}_{3}(\mathfrak{o})$.

==> background_zeta.tex <==
This section serves the purpose of introducing the tools we shall need to apply \cref{thm:A,thm:B} to the computation of representation zeta functions of almost all of the principal congruence subgroups of $\SL{3}{(\completion)}{}$. Assume that $\group=\alggroup(\completion)$ is rigid (i.e.\ its number of continuous complex $i$-dimensional irreducible representations is finite for each $i\in\N$).
%----------------------------------------------------------------------------------------------------------------------------------------------------------
%
\renewcommand{\localLielattice}{\alginf^\permiss}
%
%----------------------------------------------------------------------------------------------------------------------------------------------------------
\subsubsection{Kirillov orbit method}
\label{sec:kirillov}
We say that $\permiss\in\N$ is permissible for $\group$ when $\group^\permiss=\alggroup^\permiss(\completion)$ is potent and saturable (c.f.\ \cite[Section 2.1]{akov2013representation} for a definition of potent and saturable groups). \cite[Proposition 2.3]{akov2013representation} ensures that there is $\permiss_0\in\N$ such that $\permiss$ is permissible for $\permiss \geq \permiss_0$. Fix a permissible $\permiss\in\N$ and let $\alginf^\permiss = \padiclie(\group^\permiss)$.

First developed by Howe in \cite{how1977kirillov} in the realm of compact $p$-adic analytic groups and applied to the study of representation zeta functions of FAb compact  $p$-adic analytic groups by   Jaikin-Zapirain in \cite{zap2006zeta}, the Kirillov orbit method is a powerful tool that completely describes the irreducible representations of a group in terms of co-adjoint orbits in an $\Z_p$-Lie lattice associated with the group. The version that we  employ works with potent and saturable pro-$p$ groups and it is due to Gonzalez-Sanchez (see \cite{san2009kirillov} for a more exhaustive description).\par
We consider the Pontryagin dual of the compact abelian group $(\localLielattice,+)$
\[
\irr(\localLielattice)=\pont{\localLielattice}=\mathop{\Hom_{\Z}^{\mathrm{cont}}(\localLielattice,\C^*)},
\]
i.e.\ the group $\mathop{\Hom_{\Z}^{\mathrm{cont}}(\localLielattice,\C^*)}=\mathop{\Hom_{\Z}^{\mathrm{cont}}(\localLielattice,\prufer)}$ of continuous complex characters of the additive group $\localLielattice$, where $\prufer\cong \Q_p/\Z_p$ is the group of complex roots of unity of order a power of $p$. With each $\omega\in\irr(\localLielattice)$ we associate a biadditive bilinear form
\[
b_{\omega}:\xymatrix@R=3pt{\localLielattice \times \localLielattice \ar[r]&\prufer\\
(x,y)\ar@{|->}[r]&\omega(\comm{x}{y}{}).}
\]
We define the radical of the bilinear form $b_{\omega}$ as
\[
\rad(\omega)=\rad(b_{\omega})=\lbrace x\in\localLielattice\mid \forall\,y\in\localLielattice\,:\, b_{\omega}(x,y)=1\rbrace.
\]
The Kirillov orbit method implies that there is a one to one correspondence between orbits for the $\group^\permiss$-co-adjoint action on $\pont{\localLielattice}$ and continuous complex irreducible representations of $\group^\permiss$. In particular
\begin{equation}
\label{eq:kirillov}
\zetafunc{\group^\permiss}=\sum_{\omega\in\irr{(\localLielattice)}}\lvert \localLielattice:\rad(\omega)\rvert^{-\frac{s+2}{2}}
\end{equation}
 (c.f.\ \cite[Corollary 2.13]{san2009kirillov} and \cite[Theorem 5.2]{zap2006zeta}).
%-----------------------------------------------------------------------------------------------------------------------------------------------------------
\subsubsection{Commutator matrix and Poincar\'e series}
We give a short summary of some facts in \cite[Section 2.2, Section 3.1]{akov2013representation}. Notice that by \cref{prop:padic_lie_rings}, we may assume that $\alginf^\permiss = \pi^\permiss\lie(\alggroup)(\completion)$, therefore let $\alginf = \lie(\alggroup)(\completion)$, so that $\localLielattice = \pi^\permiss \alginf$. Let $\localfrac$ be the field of fractions of $\completion$ and set $\dim_{\localfrac} (\localfrac\otimes_{\completion} \alginf)=\dimalg$. The following lemma explains how to conveniently sort irreducible representations of the Lie lattice $\alginf$.
\begin{lem}[{\cite[Lemma 2.4]{akov2013representation}}]
\label{lem:levels}
The dual of  an $\completion$-Lie lattice $\alginf$ can be written as a disjoint union:
\[
\pont{\alginf}=\bigcup_{\level\in\N_0}^{.}\irr_\level(\alginf), \text{ where } \irr_\level(\alginf)\cong\Hom_{\completion}(\alginf, \completion/\primeideal^\level)^*.
\]
\end{lem}\noindent
For $\level\in\N_0$, an element of $ \omega\in\irr_\level(\alginf)$ is said to have level $\lev(\omega)=\level$. The sets $\irr_\level(\alginf^\permiss)$ are $\grpinf^\permiss$-invariant and therefore each irreducible representation of $\grpinf^\permiss$ corresponds to a unique co-adjoint orbit $\orbit\subseteq\irr_\level(\alginf^\permiss)$ for some level $\level\in\N_0$.\par
Thanks to this categorization of irreducible representations, it is possible to rephrase the problem of counting representations in a counting problem involving a matrix of linear forms with coefficients in $\completion$.
\subsubsection{Commutator matrix}
\label{sec:comm_matrix}
We choose an $\completion$-basis $\basis=\lbrace b_1,\dots,b_d\rbrace$ for the $\completion$-Lie lattice $\alginf$. For any $b_i,b_j\in \basis$, there are $\lambda_{i,j}^1,\dots,\lambda_{i,j}^d\in\completion$ such that
\[[b_i,b_j]=\sum_{h=1}^d \lambda_{i,j}^h b_h.\]
The coefficients $\lambda_{i,j}^h$ for $i,j,h=1,\dots,d$ are called the \emph{structure constants} of $\alginf$ with respect to $\basis$. By means of them we define the \emph{commutator matrix} of $\alginf$ as
\begin{equation}
\label{eq:comm_matrix}
\Cmatrix{\basis}{\varY}=\left( \sum_{h=1}^d \lambda_{i,j}^h Y_h\right)_{i,j}\in \Mat{d}{(\completion[\varY])}
\end{equation}
with  variables $\varY=(Y_1,\dots,Y_d)$.\par
%---------------------------------------------------------------------------------------------------------------------------------------
\begin{notation}
Let  $n_1,n_2\in\N$ and 
\[\cmatrix=(g_{ij})_{i,j=1,\dots n_1}\in\Mat{n_1}{(\completion[Y_1,\dots,Y_{n_2}])}.\] 
We write
\[
\cmatrix^{\level}=(\reduction{}{\level}(g_{ij}))_{i,j=1,\dots n_1}
\]
for the reduction $\bmod$ $\primeideal^\level$ of $\cmatrix$. When $\level=1$ we write $\overline{\cmatrix}=\cmatrix^1$.
\end{notation}
%---------------------------------------------------------------------------------------------------------------------------------------
We consider now $\tuple{w} = (w_1,\dots,w_\dimalg)\in\cone{}=(\completion^\dimalg)^*$; the matrix $\Cmatrix{\basis}{\tuple{w}}$ is an antisymmetric $\dimalg\times\dimalg$ matrix. Therefore its elementary divisors can be arranged in $\halfdim=\lfloor \dimalg/2\rfloor$ pairs $(\primeideal^{a_1},\primeideal^{a_1}),\dots,(\primeideal^{a_\halfdim},\primeideal^{a_\halfdim})$ for $0\leq a_1\leq\dots\leq a_\halfdim\in(\N_0\cup\lbrace \infty\rbrace)$ together with $\primeideal^\infty=\lbrace 0\rbrace$ if $\dimalg$ is odd. We define
\[
\nu(\Cmatrix{\basis}{\tuple{w}})=(a_1,\dots, a_\halfdim).
\]
For $\level\in\N$, let 
\begin{equation}
\label{eq:def_affine_cone}
\cone{\level}=(\cone{}+(\primeideal^\level)^{(\dimalg)})/(\primeideal^\level)^{(\dimalg)}=((\completion/\primeideal^{\level})^d)^*.
\end{equation}
Let $\tuple{w}_\level=(\reduction{}{\level}(w_1),\dots,\reduction{}{\level}(w_\dimalg))$. The valuation of the matrix $\cmatrix^\level_{\basis}(\tuple{w}_\level)$ is defined as
\[
\nu(\cmatrix^\level_{\basis}(\tuple{w}_\level))=(\min\lbrace a_i,\level\rbrace)_{i=1,\dots,\halfdim}\in\lbrace 0,1,\dots \level\rbrace^\halfdim.
\]
Recall that, in order to apply the Kirillov orbit method, we work with the congruence sublattices $\alginf^\permiss = \pi^\permiss \alginf$. We derive an $\completion$-basis for $\localLielattice$ from $\basis$ by multiplying all of its elements by $\pi^\permiss$. In other words we define a coordinate system
\begin{align*}
&\xymatrix@R=3pt{\alginf^\permiss \ar[r]&\completion^\dimalg},& \xymatrix@R=3pt{z=\sum_{i=1}^\dimalg z_i (\pi^\permiss b_i)\ar@{|->}[r]&\mathbf{z}=(z_1,\dots,z_\dimalg).}
\end{align*}
\begin{defn}
\label{def:dual_system}
We define 
\[\basis^{\sharp}=\allowbreak\lbrace b_1^{\sharp},\dots,b_\dimalg^{\sharp}\rbrace\allowbreak\subseteq \Hom_\completion(\alginf,\completion)\]
by
$b_i^{\sharp}(b_j)=\delta_{i,j}\text{ for all } i,j\in\lbrace 1,\dots,\dimalg\rbrace$.
It is a standard computation to see that $\basis^{\sharp}$ is an $\completion$-basis for $\alginf^{\sharp}=\Hom_\completion(\alginf,\completion)$. Therefore we call $\basis^{\sharp}$ the dual basis to $\basis$.
\end{defn}
We define a coordinate system on $\Hom_\completion(\alginf^\permiss,\completion)$ by shifting the dual basis $\basis^{\sharp}$:
\begin{align*}
\xymatrix@R=3pt{ \Hom_\completion(\alginf^\permiss,\completion)\ar[r]&\completion^\dimalg},& \xymatrix@R=3pt{w=\sum_{i=1}^\dimalg w_i (\pi^{-\permiss} b_i^{\sharp})\ar@{|->}[r]&\mathbf{w}=(w_1,\dots,w_\dimalg).}
\end{align*}
Since $\basis^{\sharp}$ is the dual basis of $\basis$, we have that $w(z)=\mathbf{w}\cdot\mathbf{z}$ for $z$ and $w$ as above.
\begin{defn}
\label{def:representative}
Let $\level\in\N$. We say that $w\in\Hom_\completion(\alginf^\permiss,\completion)$ is a \emph{representative} of $\omega\in\irr_\level(\alginf^\permiss)$ when $\omega$ is the image of $w$ in the natural surjection
\[
\Hom_\completion(\alginf^\permiss,\completion)^{*}\rightarrow\Hom_\completion(\alginf^\permiss,\completion/\primeideal^\level)^{*}\cong \irr_\level(\alginf^\permiss),
\]
\end{defn}
where $\irr_\level(\alginf^\permiss)$ is defined as in \cref{lem:levels}. A representative $w$ of $\omega\in\irr_\level(\alginf^\permiss)$ can be used to compute $\rad(\omega)$ as the following explains.
\begin{defn}
\label{def:rad_repr}
Let $\permiss,\level\in\N_0$. Consider $\omega\in\irr_\level(\alginf^\permiss)$ and let $w\in\mathop{\Hom_{\completion }(\alginf^{\permiss},\completion)^*}$ represent $\omega$. We define
\begin{align*}
\rad(w)&=\lbrace x\in\localLielattice\mid \forall\,y\in\alginf^\permiss\,:\, w([x,y])=0\rbrace\\
\rad_\level(w)&=\lbrace x\in\localLielattice\mid \forall\,y\in\alginf^\permiss\,:\, w([x,y])\equiv0\bmod\primeideal^\level\rbrace.
\end{align*}
\end{defn}
If $\omega\in\irr_\level(\alginf^\permiss)$ is represented by $w$, then $z\in\rad(\omega)$ if and only if $z\in\rad_\level(w)$. Expressing this in coordinates we can highlight the link between the Kirillov orbit method and the commutator matrix.
\begin{lem}
\label{lem:congruence}
Let  $\omega\in\irr_\level(\alginf^{\permiss})$ and let  $w\in\mathop{\Hom_{\completion }(\alginf^{\permiss},\completion)^*}$ be one ot its representatives. Let $\tuple{w}$ be the coordinates of $w$  in the $\completion$-basis ${\basis}^{\sharp}$ and let $\level\in\N_0$. Then for every $z\in\alginf^\permiss$ with $\basis$-coordinates $\tuple{z}\in\completion^\dimalg$ we have 
\begin{align*}
z\in\rad(w)&\iff \tuple{z}\cdot \Cmatrix{\basis}{\tuple{w}}=0,\\
z\in\rad_\level(w)&\iff \tuple{z}\cdot \pi^\permiss\Cmatrix{\basis}{\tuple{w}}\equiv0 \mod {\primeideal^{\level}}.
\end{align*}
\begin{proof}
The first double implication follows immediately from the definition of commutator-matrix, indeed for all $x,y\in\alginf^\permiss$ we have $w([x,y])=\pi^\permiss\tuple{x}\Cmatrix{\basis}{\tuple{w}} \transpose{\tuple{y}}$, where $\tuple{x}$ and $\tuple{y}$ are the coordinates of $x$ and $y$ in the basis $\pi^\permiss\basis$. The second double implication is \cite[Lemma 3.3]{akov2013representation}.
\end{proof}
\end{lem}
%
%
\subsubsection{Poincar\'e series}
\label{sec:Poin_series}
We briefly recall the definition of the Poincar\'e series associated with a matrix of linear forms and its relation with the representation zeta function of $G^\permiss$ for each permissible $\permiss\in\N$ as expressed in \cite[Section 3]{akov2013representation}. We borrow the notation from \cite[Section 3.1]{stavol2011nilpotent}.\par
Let $\cmatrix\in\Mat{\dimalg}{(\completion[\varY])}$ be an antisymmetric matrix of linear forms in $f$ variables. Let $I=\lbrace i_1,\dots,i_\lastindex \rbrace_{<}\subseteq [\halfdim-1]_0$. We impose $i_0=0$ and $i_{\lastindex+1}=\halfdim$ and we write 
\[\mu_j=i_{j+1}-i_j\]
with $j\in[\lastindex]_0$ (so $\mu_\lastindex = \halfdim - i_\lastindex$). For $\mathbf{r}_I=(r_{1},\dots,r_{\lastindex})\in \N^{\lvert I\rvert}$, we set $N=\sum_{j=1}^\lastindex r_j$. The \emph{Poincar\'e series of $\cmatrix$} is
\begin{equation*}
\pseries{\mathcal{R}}(s)=\sum_{\stackrel{I\subseteq [\halfdim-1]_0}{I=\lbrace i_1,\dots,i_\lastindex \rbrace_{<}}}\sum_{\mathbf{r}_I\in\N^{\lvert I\rvert}} \lvert \pcoeff{I}{(\cmatrix)}\rvert\,q^{-s\sum_{j=1}^\lastindex r_j(\halfdim-i_j)},
\end{equation*}
where
\begin{multline*}
\pcoeff{I}{(\cmatrix)}= \lbrace \tuple{w}\in \cone{N}\mid \nu(\cmatrix(\tuple{w}))=(\underbrace{0,\dots,0}_{\mu_\lastindex},\underbrace{r_{\lastindex},\dots,r_{\lastindex}}_{\mu_{\lastindex-1}},\\
			\underbrace{r_{\lastindex} + r_{\lastindex-1} ,\dots,r_{\lastindex} + r_{\lastindex-1} }_{\mu_{\lastindex-2}}%
					\dots%
						,\underbrace{N,\dots,N}_{\mu_0})\in \N_0^\halfdim\rbrace.
\end{multline*}
Let $\cmatrix=\cmatrix_{\basis}$ (in particular we have $f=\dimalg$). We set
\begin{equation}
\label{eq:p_coeff_card}
\pcoeffCard{I}{(\alginf)}=\lvert \pcoeff{I}{(\cmatrix)}\rvert\\
\end{equation}
This is clearly well defined as changing basis for $\alginf$ results in a linear invertible substitution of variables in the linear forms constituting the entries of $\cmatrix$. As a consequence we can define
\begin{equation}
\label{eq:Poin_series}
\pseries{\alginf}(s)=\sum_{\stackrel{I\subseteq [\halfdim-1]_0}{I=\lbrace i_1,\dots,i_\lastindex \rbrace_{<}}}\sum_{\mathbf{r}_I\in\N^{\lvert I\rvert}}\pcoeffCard{I}{(\alginf)}
\,
q^{-s\sum_{j=1}^\lastindex r_j(\halfdim-i_j)}.
\end{equation}
\begin{rem}
\label{rem:rank_mod_p}
Let $w\in\pcoeff{I}{(\cmatrix)}$, then the definition of $\pcoeff{I}{(\cmatrix)}$ entails that 
\[{\rk}_{\qfield} \overline{\cmatrix(w)} = \halfdim-i_\lastindex
\]
\todo{modify notation for reduction mod p}
where $\overline{\cmatrix(w)}$ is the reduction $\bmod\,\primeideal$ of $\cmatrix(w)$.
\end{rem}
The following illustrates the relation between the representation zeta function and the Poincar\'e series.
\begin{prop}[{\cite[Proposition 3.1]{akov2013representation}}]
\label{prop:zeta_poinc}
For all $\permiss$ that are permissible for $\group$
\[
\zetafunc{G^\permiss}=q^{\dimalg\cdot \permiss}\,\mathcal{P}_{\alginf}(s+2).
\]
\end{prop}
